Convex Hulls under Uncertainty

We study the convex-hull problem in a probabilistic setting, motivated by the need to handle data uncertainty inherent in many applications, including sensor databases, location-based services and computer vision. In our framework, the uncertainty of each input site is described by a probability distribution over a finite number of possible locations including a \emph{null} location to account for non-existence of the point. Our results include both exact and approximation algorithms for computing the probability of a query point lying inside the convex hull of the input, time-space tradeoffs for the membership queries, a connection between Tukey depth and membership queries, as well as a new notion of $\some$-hull that may be a useful representation of uncertain hulls.

==> figs/tex/x/ocomp.tex <==
\definecolor{a0a0a4}{RGB}{160,160,164}
\definecolor{000000}{RGB}{0,0,0}
\definecolor{808080}{RGB}{128,128,128}
\begin{tikzpicture}[x=1cm,y=1cm]
\clip (15,0) rectangle (18,3);
%% tikzlabel;
\node [color=000000,inner sep=0.5pt,above,shift={(0,3pt)}] at (0.49296,0.00762142) {$\circled{$\GroupX{2}$}$};
%% tikzlabel;
\node [color=000000,inner sep=0.5pt,below right,shift={(3pt,-3pt)}] at (1.37078,0.945937) {$\mpt$};
%% tikzlabel;
\node [color=000000,inner sep=0.5pt,above,shift={(0,3pt)}] at (2.45777,0.885647) {$\circled{$\GroupX{1}$}$};
%% tikzlabel;
\node [color=000000,inner sep=0.5pt,right,shift={(4pt,0)}] at (1.92125,2.11751) {$\siX{i}$};
%% tikzlabel;
\node [color=000000,inner sep=0.5pt,above left,shift={(-3pt,3pt)}] at (6.06623,2.36556) {$\siX{2}$};
%% tikzlabel;
\node [color=000000,inner sep=0.5pt,above left,shift={(-3pt,3pt)}] at (5.51536,1.86844) {$\siX{1}$};
%% tikzlabel;
\node [color=000000,inner sep=0.5pt,above right,shift={(3pt,3pt)}] at (6.60369,2.00193) {$...$};
%% tikzlabel;
\node [color=000000,inner sep=0.5pt,right,shift={(3pt,0)}] at (11.4742,1.51824) {$\mpt$};
%% tikzlabel;
\node [color=000000,inner sep=0.5pt,below right,shift={(3pt,-3pt)}] at (6.49617,1.36459) {$\mpt$};
%% tikzlabel;
\node [color=000000,inner sep=0.5pt,below right,shift={(3pt,-3pt)}] at (6.28795,0.785994) {$...$};
%% tikzlabel;
\node [color=000000,inner sep=0.5pt,above,shift={(0,3pt)}] at (11.4204,0.107486) {$\circled{$\SGroup'$}$};
%% tikzlabel;
\node [color=000000,inner sep=0.5pt,below left ,shift={(-3pt,-3pt)}] at (5.51539,0.960659) {$\siX{n}$};
%% tikzlabel;
\node [color=000000,inner sep=0.5pt,left,shift={(-3pt,0)}] at (10.8293,2.37814) {$\siX{i-1}$};
%% tikzlabel;
\node [color=000000,inner sep=0.5pt,right,shift={(3pt,0)}] at (12.0385,2.37814) {$\siX{i}$};
%% tikzlabel;
\node [color=000000,inner sep=0.5pt,right,shift={(3pt,0)}] at (16.3098,1.23982) {$\mpt$};
%% tikzlabel;
\node [color=000000,inner sep=0.5pt,above left,shift={(-3pt,3pt)}] at (16.6013,1.84811) {$\f_j$};
%% tikzlabel;
\node [color=000000,inner sep=0.5pt,above,shift={(0,3pt)}] at
(15.4861,1.92414) {$\siX{i}$};
%% tikzlabel;
\node [color=000000,inner sep=0.5pt,above,shift={(0,3pt)}] at
(17.1462,0.568163) {$\circled{$\GroupX{1}$}$};
%% tikzlabel;
\node [color=000000,inner sep=0.5pt,right,shift={(3pt,0)}] at
(16.8927,2.4564) {$\siX{j}$};
%% segment;
\draw[color=a0a0a4,line width=1,dotted] (-2.14531,0.945937) -- (1.37078,0.945937);
%% line;
%% segment;
\draw[color=a0a0a4,line width=1,dotted] (0.637247,-0.615251) -- (2.56193,3.48108);
%% segment;
\draw[color=a0a0a4,line width=1,dotted] (15.3266,-0.812143) -- (17.5569,3.84246);
%% line;
%% segment;
\draw[color=a0a0a4,line width=1,dotted] (4.7697,1.36459) -- (8.49141,1.36459);
%% line;
%% vector;
%% line;
%% vector;
%% segment;
\draw[color=000000,line width=1] (1.92125,2.11751) -- (1.37078,0.945937);
%% vector;
%% segment;
\draw[color=808080,line width=1,densely dashed] (6.49617,1.36459) -- (6.28795,0.785994);
%% segment;
\draw[color=a0a0a4,line width=1,dotted] (12.8309,-0.290739) -- (10.1622,3.2677);
%% line;
%% segment;
\draw[color=808080,line width=1,densely dashed] (6.49617,1.36459) -- (6.60369,2.00193);
%% segment;
\draw[color=808080,line width=1,densely dashed] (6.49617,1.36459) -- (5.51539,0.960659);
%% segment;
\draw[color=a0a0a4,line width=1,dotted] (12.6337,3.28505) -- (10.3188,-0.24235);
%% segment;
\draw[color=808080,line width=1,densely dashed] (6.06623,2.36556) -- (6.49617,1.36459);
%% segment;
\draw[color=808080,line width=1,densely dashed] (5.51536,1.86844) -- (6.49617,1.36459);
%% segment;
\draw[color=000000,line width=1] (16.3098,1.23982) -- (16.8927,2.4564);
%% line;
%% point;
\path [fill=000000] (16.8927,2.4564) circle (1.5pt);
%% point;
%% point;
\path [fill=000000] (6.06623,2.36556) circle (1.5pt);
%% point;
\path [fill=000000] (6.49617,1.36459) circle (1.5pt);
%% point;
\path [fill=000000] (5.51536,1.86844) circle (1.5pt);
%% point;
%% point;
%% point;
\path [fill=000000] (1.37078,0.945937) circle (1.5pt);
%% point;
%% point;
%% point;
%% point;
\path [fill=000000] (1.92125,2.11751) circle (1.5pt);
%% point;
%% point;
%% point;
%% point;
\path [fill=000000] (5.51539,0.960659) circle (1.5pt);
%% point;
%% point;
%% point;
%% point;
%% point;
\path [fill=000000] (12.0385,2.37814) circle (1.5pt);
%% point;
%% point;
\path [fill=000000] (11.4742,1.51824) circle (1.5pt);
%% point;
%% point;
%% point;
\path [fill=000000] (10.8293,2.37814) circle (1.5pt);
%% point;
%% point;
%% point;
%% point;
%% point;
%% point;
\path [fill=000000] (16.3098,1.23982) circle (1.5pt);
%% point;
\path [fill=000000] (15.4861,1.92414) circle (1.5pt);
\end{tikzpicture}


==> figs/tex/x/old_ver/ocomp.tex <==
\definecolor{a0a0a4}{RGB}{160,160,164}
\definecolor{000000}{RGB}{0,0,0}
\definecolor{808080}{RGB}{128,128,128}
\begin{tikzpicture}[x=1cm,y=1cm]
\clip (15,0) rectangle (18,3);
%% tikzlabel;
\node [color=000000,inner sep=0.5pt,above,shift={(0,3pt)}] at (0.49296,0.00762142) {$\circled{$\GroupX{2}$}$};
%% tikzlabel;
\node [color=000000,inner sep=0.5pt,below right,shift={(3pt,-3pt)}] at (1.37078,0.945937) {$\mpt$};
%% tikzlabel;
\node [color=000000,inner sep=0.5pt,above,shift={(0,3pt)}] at (2.45777,0.885647) {$\circled{$\GroupX{1}$}$};
%% tikzlabel;
\node [color=000000,inner sep=0.5pt,right,shift={(4pt,0)}] at (1.92125,2.11751) {$\siX{i}$};
%% tikzlabel;
\node [color=000000,inner sep=0.5pt,above left,shift={(-3pt,3pt)}] at (6.06623,2.36556) {$\siX{2}$};
%% tikzlabel;
\node [color=000000,inner sep=0.5pt,above left,shift={(-3pt,3pt)}] at (5.51536,1.86844) {$\siX{1}$};
%% tikzlabel;
\node [color=000000,inner sep=0.5pt,above right,shift={(3pt,3pt)}] at (6.60369,2.00193) {$...$};
%% tikzlabel;
\node [color=000000,inner sep=0.5pt,right,shift={(3pt,0)}] at (11.4742,1.51824) {$\mpt$};
%% tikzlabel;
\node [color=000000,inner sep=0.5pt,below right,shift={(3pt,-3pt)}] at (6.49617,1.36459) {$\mpt$};
%% tikzlabel;
\node [color=000000,inner sep=0.5pt,below right,shift={(3pt,-3pt)}] at (6.28795,0.785994) {$...$};
%% tikzlabel;
\node [color=000000,inner sep=0.5pt,above,shift={(0,3pt)}] at (11.4204,0.107486) {$\circled{$\SGroup'$}$};
%% tikzlabel;
\node [color=000000,inner sep=0.5pt,below left ,shift={(-3pt,-3pt)}] at (5.51539,0.960659) {$\siX{n}$};
%% tikzlabel;
\node [color=000000,inner sep=0.5pt,left,shift={(-3pt,0)}] at (10.8293,2.37814) {$\siX{i-1}$};
%% tikzlabel;
\node [color=000000,inner sep=0.5pt,right,shift={(3pt,0)}] at (12.0385,2.37814) {$\siX{i}$};
%% tikzlabel;
\node [color=000000,inner sep=0.5pt,right,shift={(3pt,0)}] at (16.3098,1.23982) {$\mpt$};
%% tikzlabel;
\node [color=000000,inner sep=0.5pt,above left,shift={(-3pt,3pt)}] at (16.6013,1.84811) {$\f_j$};
%% tikzlabel;
\node [color=000000,inner sep=0.5pt,above,shift={(0,3pt)}] at
(15.4861,1.92414) {$\siX{i}$};
%% tikzlabel;
\node [color=000000,inner sep=0.5pt,above,shift={(0,3pt)}] at
(17.1462,0.568163) {$\circled{$\GroupX{1}$}$};
%% tikzlabel;
\node [color=000000,inner sep=0.5pt,right,shift={(3pt,0)}] at
(16.8927,2.4564) {$\siX{j}$};
%% segment;
\draw[color=a0a0a4,line width=1,dotted] (-2.14531,0.945937) -- (1.37078,0.945937);
%% line;
%% segment;
\draw[color=a0a0a4,line width=1,dotted] (0.637247,-0.615251) -- (2.56193,3.48108);
%% segment;
\draw[color=a0a0a4,line width=1,dotted] (15.3266,-0.812143) -- (17.5569,3.84246);
%% line;
%% segment;
\draw[color=a0a0a4,line width=1,dotted] (4.7697,1.36459) -- (8.49141,1.36459);
%% line;
%% vector;
%% line;
%% vector;
%% segment;
\draw[color=000000,line width=1] (1.92125,2.11751) -- (1.37078,0.945937);
%% vector;
%% segment;
\draw[color=808080,line width=1,densely dashed] (6.49617,1.36459) -- (6.28795,0.785994);
%% segment;
\draw[color=a0a0a4,line width=1,dotted] (12.8309,-0.290739) -- (10.1622,3.2677);
%% line;
%% segment;
\draw[color=808080,line width=1,densely dashed] (6.49617,1.36459) -- (6.60369,2.00193);
%% segment;
\draw[color=808080,line width=1,densely dashed] (6.49617,1.36459) -- (5.51539,0.960659);
%% segment;
\draw[color=a0a0a4,line width=1,dotted] (12.6337,3.28505) -- (10.3188,-0.24235);
%% segment;
\draw[color=808080,line width=1,densely dashed] (6.06623,2.36556) -- (6.49617,1.36459);
%% segment;
\draw[color=808080,line width=1,densely dashed] (5.51536,1.86844) -- (6.49617,1.36459);
%% segment;
\draw[color=000000,line width=1] (16.3098,1.23982) -- (16.8927,2.4564);
%% line;
%% point;
\path [fill=000000] (16.8927,2.4564) circle (1.5pt);
%% point;
%% point;
\path [fill=000000] (6.06623,2.36556) circle (1.5pt);
%% point;
\path [fill=000000] (6.49617,1.36459) circle (1.5pt);
%% point;
\path [fill=000000] (5.51536,1.86844) circle (1.5pt);
%% point;
%% point;
%% point;
\path [fill=000000] (1.37078,0.945937) circle (1.5pt);
%% point;
%% point;
%% point;
%% point;
\path [fill=000000] (1.92125,2.11751) circle (1.5pt);
%% point;
%% point;
%% point;
%% point;
\path [fill=000000] (5.51539,0.960659) circle (1.5pt);
%% point;
%% point;
%% point;
%% point;
%% point;
\path [fill=000000] (12.0385,2.37814) circle (1.5pt);
%% point;
%% point;
\path [fill=000000] (11.4742,1.51824) circle (1.5pt);
%% point;
%% point;
%% point;
\path [fill=000000] (10.8293,2.37814) circle (1.5pt);
%% point;
%% point;
%% point;
%% point;
%% point;
%% point;
\path [fill=000000] (16.3098,1.23982) circle (1.5pt);
%% point;
\path [fill=000000] (15.4861,1.92414) circle (1.5pt);
\end{tikzpicture}

